Subjective Evaluation of Deep Learning Models for Symbolic Music Composition

Deep learning models are typically evaluated to measure and compare their performance on a given task. The metrics that are commonly used to evaluate these models are standard metrics that are used for different tasks. In the field of music composition or generation, the standard metrics used in other fields have no clear meaning in terms of music theory. In this paper, we propose a subjective method to evaluate AI-based music composition systems by asking questions related to basic music principles to different levels of users based on their musical experience and knowledge. We use this method to compare state-of-the-art models for music composition with deep learning. We give the results of this evaluation method and we compare the responses of each user level for each evaluated model.

==> sections/attributes.tex <==
\section{Evaluation of AI-based Music Composition Systems} \label{sec:attributes}


\subsection{Symbolic Music Generation}
AI-based music composition is normally evaluated with metrics such as the accuracy or the perplexity. DL models are also compared with their loss function. The loss function can give a general idea of how the model generalizes in a particular dataset, but there is a lack of standard method to evaluate and properly compare AI-based music composition models due to the difficulties of measuring music. Accuracy metrics cannot explain or measure all the music intricacies that depend on the music basic principles (see section \ref{sec:basic}). We can distinguish between subjective and objective evaluation methods. In one hand, there have been done listening tests \cite{musicvae}, \cite{deepbach} that are too general to evaluate the music that a model generates. In the other hand, there have been proposed some objective metrics \cite{survey}, \cite{yang2020evaluation}.

Symbolic music basic principles are: melody, harmony, form or structure and texture. There are other music principles that are not in the scope of this work because they are not sheet or symbolic music principles but they are more related to the performance such as timbre, dynamics or effects. In Table \ref{tab:survey} we tag the survey questions to these principles: melody (M), harmony (H) and rhythm (R).

